Improving DBMS Scheduling Decisions with Fine-grained Performance Prediction on Concurrent Queries -- Extended

Query scheduling is a critical task that directly impacts query performance in database management systems (DBMS). Deeply integrated schedulers, which require changes to DBMS internals, are usually customized for a specific engine and can take months to implement. In contrast, non-intrusive schedulers make coarse-grained decisions, such as controlling query admission and re-ordering query execution, without requiring modifications to DBMS internals. They require much less engineering effort and can be applied across a wide range of DBMS engines, offering immediate benefits to end users. However, most existing non-intrusive scheduling systems rely on simplified cost models and heuristics that cannot accurately model query interactions under concurrency and different system states, possibly leading to suboptimal scheduling decisions. This work introduces IconqSched, a new, principled non-intrusive scheduler that optimizes the execution order and timing of queries to enhance total end-to-end runtime as experienced by the user query queuing time plus system runtime. Unlike previous approaches, IconqSched features a novel fine-grained predictor, Iconq, which treats the DBMS as a black box and accurately estimates the system runtime of concurrently executed queries under different system states. Using these predictions, IconqSched is able to capture system runtime variations across different query mixes and system loads. It then employs a greedy scheduling algorithm to effectively determine which queries to submit and when to submit them. We compare IconqSched to other schedulers in terms of end-to-end runtime using real workload traces. On Postgres, IconqSched reduces end-to-end runtime by 16.2%-28.2% on average and 33.6%-38.9% in the tail. Similarly, on Redshift, it reduces end-to-end runtime by 10.3%-14.1% on average and 14.9%-22.2% in the tail.

==> timeline.tex <==
\section{Timeline}
We are currently aiming at submitting to the VLDB 8.1 deadline. 
In the following, we list a set of must-do, nice-to-have, and future works. 

\noindent \textbf{Must-dos:}

\begin{itemize}
    \item Simulate a particular scenario to showcase how our scheduler works. 
    \item Simulate two real Snowset workload traces on the IMDB dataset (by 6.1).
    \item Run our model and baselines on real workload traces (by 7.1).
    \item Tuning the performance of our model on these two traces on Postgres, Redshift, and Aurora (by 7.15).
    \item Conduct the scalability experiments: vary 2-20 clients issuing queries in a close-loop and test our performance (by 6.15).
    \item Conduct the ablation study: measuring overhead, comparing accuracy with naive and GNN baselines, and testing the optimality of our scheduling algorithm (by 7.15).
    \item Finish paper writing (by 8.1)
\end{itemize}

\noindent \textbf{Nice-to-haves:}

\begin{itemize}
    \item If our estimator is not accurate enough, try the following: 1) adding pre-execution info to training and testing, 2) adding query exiting info, 3) exploring better separation techniques, and 4) trying graph featurization (by 7.15).
    \item If our scheduler is ineffective, design a dynamic programming algorithm (by 7.15). We are very likely to have this algorithm to increase the novelty of this paper. 
    \item Conduct robustness experiment, e.g., train on <5 clients traces and test on >5 client traces, including data update \& workload shift into consideration. 
\end{itemize}

\noindent \textbf{Future works:}
\begin{itemize}
    \item Cost model overhead issue: a stage model approach, and ignoring short-running queries
    \item Use simple model to extrapolate the learned LTSM: using classification of query types.
    \item Consider interaction between analytical and transcational queries. Can the scheduler work for transactions?
    \item Better engineering and open source software to benefit more people.
    \item Study the effect of using true cardinality, thus motivating the need of cardinality corrector.
\end{itemize}

\subsection{To-dos before next PI meetings}
Time: Jun 18th 10pm

\begin{itemize}
    \item Tune the workload trace
    \item Retrain LSTM on new queries
    \item Implement k-step look-ahead method for scoring
    \item Review literature on batch query scheduling
    \item New performance on real workload trace
    \item Discuss thesis proposal and Amazon part-time
\end{itemize}

Time: Jul 2nd 10pm

\begin{itemize}
    \item Tune performance on real workload and scalability trace
    \item Discuss the part-time CPT application
\end{itemize}

Time: Jul 16th 10pm

\begin{itemize}
    \item Design and implement new batching scheduling algo if necessary
    \item Tune new performance on real workload and scalability trace
    \item Get reasonable baseline performance
\end{itemize}

Time: Jul 30th 10pm

\begin{itemize}
    \item Finish all the remaining experiment
    \item Finish paper writing
\end{itemize}

\subsection{To-dos before next PI meetings}

Potential baselines to compare with.

Concurrent query performance prediction:

\begin{itemize}
    \item Contender: A Resource Modeling Approach for Concurrent Query Performance Prediction.
    \item Query Performance Prediction for Concurrent Queries using Graph Embedding.
    \item Performance Prediction
for Concurrent Database Workloads (bal).
\end{itemize}

Client-side scheduler \& admission controller:

\begin{itemize}
    \item Interaction-aware scheduling of report-generation workloads (Qshuffler).
    \item Fair, Effective, Efficient and Differentiated Scheduling in an Enterprise Data Warehouse.
    \item Performance Prediction
for Concurrent Database Workloads (bal).
\end{itemize}

